(Re)construing Meaning in NLP

Human speakers have an extensive toolkit of ways to express themselves. In this paper, we engage with an idea largely absent from discussions of meaning in natural language understanding--namely, that the way something is expressed reflects different ways of conceptualizing or construing the information being conveyed. We first define this phenomenon more precisely, drawing on considerable prior work in theoretical cognitive semantics and psycholinguistics. We then survey some dimensions of construed meaning and show how insights from construal could inform theoretical and practical work in NLP.

==> nertstyle.tex <==

\section{Working in drafts}

\paragraph{Notes.}
In nert.sty there are commands for you to leave notes with your initials: \nss{Nathan} \ttor{Tiago} \st{Sean} \nc{Nancy}. At submission time, you can hide them by uncommenting \verb|\renewcommand{\nertcomment}[4]{\unskip}| before the start of the document.

You can also use Overleaf's commenting feature, but these comments will not be printed in the draft.

\paragraph{Document versions.}
There are macros you can use to turn certain content on or off
depending on a particular stage in the lifecycle of the paper:
\begin{itemize}
    \item \verb|\draftversion{...}| for content that goes in internal drafts, \verb|\subversion{...}| for the official submission, \verb|\finalversion{...}| for the final version
    \item \verb|\anonversion{...}| for when the paper is anonymized, 
    \verb|\nonanonversion{...}| for when it isn't
    \item Length alternatives for working within a page limit:\\ \verb|\shortversion{...}|, \verb|\longversion{...}|, \verb|\shortlong{short...}{long...}|, \verb|\considercutting{...}|
\end{itemize}
Edit the macro definitions in nert.sty to control which will display 
their contents and which will be hidden
(they are independent of \verb|\aclfinalcopy|).

\section{Bibliography and citations}\label{sec:bib}

\paragraph{Bibliography.}
I recommend creating a fresh .bib file specifically for each paper you write. 
If you curate citation info in a reference manager, you can export the relevant citations as \BibTeX{} 
(Zotero users, see \url{https://gist.github.com/nschneid/2257875} for customizing 
how \BibTeX{} entries are created).
The \href{https://www.aclweb.org/anthology/}{ACL Anthology} generally has high-quality .bib entries. 
Entries should include URLs where possible.

By default, only papers cited at least once will appear under \textbf{References}.\footnote{\label{fn:emptybib}If your paper has an empty .bib file or no citations, compiling will trigger the error \texttt{Something's wrong-{}-perhaps a missing \textbackslash item}.}

Pay special attention to \textbf{capitalization in titles}: 
by default, the ACL stylesheet will lowercase all characters except the first in the title.

\paragraph{Citations.}
Citation commands are based on the \href{http://tug.ctan.org/macros/latex/contrib/natbib/natbib.pdf}{\texttt{natbib}} package, including 
\verb|\citep| for parenthesized citations (authors in parentheses),
\verb|\citet| for textual citations (authors before parentheses), 
\verb|\citeposs| for textual citations with a possessive author, and
\verb|\citealp| for citations without any parentheses.
Use capitalized equivalents (e.g., \verb|\Citet|) at the beginning 
of a sentence. Optional square brackets specify extra material to put at the beginning or end within the parentheses.
For example:

\begin{quote}
\Citet{blodgett-18} provided a technique that has been adapted in subsequent work on English \citep{schneider-18,prange-19} and extended to other languages \citep[e.g.,][]{zhu-19}.
Current practice is detailed in the latest guidelines \citep[pp.~77--78]{snacs}.
\Citeposs{manning-19} system adopts a different approach.
\end{quote}

\section{Cross-references}\label{sec:xref}

Units of your document---including sections, numbered linguistic examples, 
tables, and figures---can be labeled for cross-referencing. 
This is advisable in case the structure of your document changes.
It is recommended to use consistent prefixes in your labels: 
\verb|\label{fig:myfigure}|, \verb|\label{tab:mytable}|, 
\verb|\label{sec:mysection}|, \verb|\label{ex:myexample}|, 
\verb|\label{fn:myfootnote}|, etc.\footnote{\label{fn:captions}Note that 
table and figure labels must go inside or after the \texttt{\textbackslash caption} command.}

{\bfseries Please use the \verb|\cref| command (based on the \href{http://tug.ctan.org/macros/latex/contrib/cleveref/cleveref.pdf}{\texttt{cleveref}} package) for cross-references.}
It will automatically display the number with the word ``figure'' or ``table'', 
the section symbol (\S), or other formatting as appropriate. 
It supports a comma-separated list of multiple cross-references of the same type.
Capitalize as \verb|\Cref| at the beginning of a sentence.
For example:

\begin{quote}
\Cref{fn:captions} provides an important addendum. Cross-references and linguistic examples are discussed herein (\cref{sec:xref,sec:ling}).
\end{quote}

\section{Linguistic examples}\label{sec:ling}

For most purposes, the \href{http://texdoc.net/texmf-dist/doc/latex/linguex/linguex-doc.pdf}{\texttt{linguex}} package provides the simplest commands 
for numbered linguistic examples. They look like this:

\ex.\label{ex:first} Here is an example.

\ex.\label{ex:second} Here is another one.
    \a. It has a subpart.
    \b.\label{ex:subpart2} And a subsequent subpart.
        \a.\label{ex:subsubpart} with its own subpart
        \z.
    \b.\label{ex:subpart3} And so on.
    \b.\label{ex:subpart4} And so forth.

The cross-referencing commands (\cref{sec:xref}) will work: \cref{ex:second}, \cref{ex:subsubpart}, \cref{ex:subpart2,ex:subpart3,ex:subpart4}. 
Glosses are also supported; see the \href{http://mirrors.ctan.org/macros/latex/contrib/linguex/doc/linguex-doc.pdf}{package documentation} for details.

nert.sty defines a few macros for linguistic notation: 
\sst{Supersense}, \psst{SNACSSupersense}, \rf{Role}{Function}; 
boxed numbers \svar{1}, \SVAR{2}; etc.

\section{Style}

There are many places you can go for \LaTeX{} typesetting tips. 
Of particular note:

\begin{itemize}
    \item Look carefully at ``quotes'' to ensure they're curly and going in the right direction. ''BAD"
    \item Footnotes go \emph{after} post-word punctuation like periods and commas. 
    It feels illogical,\footnote{not logical} 
    but the other way looks ugly.
    \item Note the placement of periods in the following abbreviations:
    \begin{quote}
    e.g. `for example, \dots'\\
    i.e. `that is, \dots'\\
    cf. `compare'
    \end{quote}
    These abbreviations should always precede the thing they are modifying.
    \item If not followed by a comma or colon, non-sentence-final abbreviations including 
    \emph{e.g.}, \emph{i.e.}, \emph{cf.}, \emph{p.}, \emph{vs.}, and \emph{etc.}\ 
    should be separated from the next word in the sentence by a tilde (\texttt{\tat}) or backslash+space.\footnote{The difference between these is that the tilde prevents a line break. The tilde is ideal for \emph{e.g.}, \emph{i.e.}, \emph{cf.}, and \emph{p.}, which are essentially prefixes and should not appear at the end of a line.} This is to prevent \LaTeX{} from thinking it's the end of a sentence and adding a bit of extra space.\footnote{Because an end-of-sentence period may be followed by a close parenthesis or close quote, this policy applies for parenthesized or quoted ``abbrevs.''\ as well.} Compare:
    
    \begin{quote}
    E.g. preps. (and postps.) are the best (UNEVENLY SPACED)
    
    E.g.~preps.\ (and postps.)\ are the best (EVENLY SPACED)
    \end{quote}
    \item Dashes are wider than hyphens and serve a different function. 
    For numeric ranges, use \verb|--|, which typesets an \emph{en~dash}. 
    For phrase separation similar to a colon or parentheses, use \verb|---|, which typesets an \emph{em~dash}. In NERT style these are not separated by spaces:
    
    \begin{quote}
    pp.~5--10
    \end{quote}
    \begin{quote}
    ADPs---e.g., \p{in}, \p{at}, and \p{for}---are highly frequent in English.
    \end{quote}
    \item For textual lists of three or more items, NERT style uses the serial (Oxford) comma before the conjunction, as in the above example.
    \item If not in an equation or formula, typeset the numerical part outside of math mode, but numerical modifier symbols \emph{in} math mode to distinguish them from textual punctuation:
    
    \begin{quote}
    between $-$86.3 and $+$92.7
    \end{quote}
    
    Use math symbol \verb|\approx|, not \verb|~|, for approximate quantities:
    
    \begin{quote}
    $\approx$100 minutes
    \end{quote}
\end{itemize}


